Practical Dataset Distillation Based on Deep Support Vectors

Conventional dataset distillation requires significant computational resources and assumes access to the entire dataset, an assumption impractical as it presumes all data resides on a central server. In this paper, we focus on dataset distillation in practical scenarios with access to only a fraction of the entire dataset. We introduce a novel distillation method that augments the conventional process by incorporating general model knowledge via the addition of Deep KKT (DKKT) loss. In practical settings, our approach showed improved performance compared to the baseline distribution matching distillation method on the CIFAR-10 dataset. Additionally, we present experimental evidence that Deep Support Vectors (DSVs) offer unique information to the original distillation, and their integration results in enhanced performance.

==> sec/original_method.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
\subsection{Deep Support Vectors}
\hh{ 기존의 svm의 목적은 data들을 class에 맞게 가장 효과적으로 구분할 수 있는 hyperplane을 찾는것이다. 이때 이 hyperplane은 data들간의 margin을 최대화하도록 만들어지며, margin값을 최대화하는데에 결정적인 영향을 미치는 class들의 boundary에 있는 data들을 support vector들이라고 정의한다. SVM이 margin을 최대화하면서 classifier의 역할을 수행해야하므로 SVM은 아래의 kkt(Karush–Kuhn–Tucker) 조건을 만족시켜야한다. 
 %
\begin{equation}
\begin{aligned}
&\text{Primal feasibility:} && \forall i,\ y_i \tilde{w}^T \tilde{x}_i \geq 1, \\
&\text{Dual feasibility:} && \forall i,\ \alpha_i \geq 0, \\
&\text{Complementary slackness}: &&  \alpha_i \left( y_i \tilde{w}^T \tilde{x}_i - 1 \right) = 0, \\
&\text{Stationarity:} && \tilde{w} =   \sum_{i=1}^n \alpha_i y_i \tilde{x}_i .
\end{aligned}
\label{eq:KKT}
\end{equation}
%
이준후et al은 기존 linearly seperable data에 classifier로 쓰인 SVM을 nonlinear한 deep learning model $\Phi(\cdot; \theta^*)$  로 확장하였으며 support vector의 역할을 하는 Deep Support Vector들을 새로히 정의하였다. deep learning model $\Phi(\cdot; \theta^*)$의 목적은 주어진 데이터에 대하여 정확하게 classify하는것으로, 전체 logit $\Phi(x_i; \theta) = [\Phi_1(x_i; \theta), \cdots, \Phi_C(x_i; \theta)]^T \in \mathbb{R}^C$ 중 정답 class에 해당하는 logit $\Phi_{y_i}(x_i; \theta)$ 을 최대화하는 것을 목적으로 한다. 이는 아래 cross entropy loss를 minimize하는것과 같고, negative loss를 margin이라고 가정하면 margin을 maximize하는것으로도 볼 수 있다.  
\begin{equation}
-L_{ce} = \Phi_{y_i}(x_i; \theta^*) - \log \sum_{c=1}^C \exp (\Phi_{c}(x_i; \theta^*)),
\label{eq:primal_ce}
\end{equation}   
Deep learning model에서의 margin에 해당하는 $-L(\Phi(x_i; \theta^*), y_i)$과 기존의 binary classification SVM maximize해야하는 margin $y_i \tilde{w}^T \tilde{x}_i $ 사이의 analogy를 찾을 수 있으며 이때 SVM에서의 $y_i \tilde{x}_i (=\nabla_{\tilde{w}} (y_i\tilde{w}^T\tilde{x}_i))$ 는 Deep learning model에서 $-\nabla_\theta^* L(\Phi(x_i; \theta^*), y_i)$로 대응이 된다. 이러한 대응관계로 SVM의 KKT조건에서 Deep Learning model에 해당하는 DeepKKT조건으로 바꿀 수 있다. 다만 저차원에서 정의되는 SVM과 달리 deep learning model들은 고차원 공간에서 동작하므로 DSV들을 data manifold로 가게하는 manifold condition을 추가하였다. DKKT condition은 아래와 같다.

%
\begin{equation*} \label{eq:DeepKKT}
\begin{aligned}
&\text{Primal feasibility:} && 
\forall\, i \in \mathcal{I}, \quad \argmax_c\; \Phi_c (x_i; \theta^*) = y_i \\
%\jh{\forall argmax \Phi(X_i; \theta^*) = y_i}, \\%  \nj{\Phi_{y_i}(x_i; \theta^*) \geq 1}\\ 
&\text{Dual feasibility:} && \forall\, i \in \mathcal{I}, \quad \lambda_i \geq 0, \\
% &\text{CS condition:} 
%&\text{slackness:} 
% && \forall\, i \in \mathcal{I}, \quad % \in [n],
% \ \nj{\lambda_i (y_i \Phi(x_i; \theta^*) - 1) = 0}, \\
&\text{Stationarity:} && \theta^* = -\sum_{i=1}^n \lambda_i \nabla_{\theta} \mathcal{L}(\Phi(x_i; \theta^*), y_i), \\
&\text{Manifold:} && \forall\, i \in \mathcal{I}, \quad x_i \in \mathcal{M}. 
\end{aligned}
\end{equation*}
%
}
\nj{notation에 대한 설명 필요.}
\hh{DSV들은 decision boundary에 대한 정보를 가지고 있기도 하지만 dataset 자체의 representation이기도 하다. 따라서 dataset condensation에서의 role 또한 수행할 수 있으며 실제로 기존의 condensation method와 비교했을 때도 비슷한 성능이 나옴을 확인할 수 있다. Training dataset에 대한 접근이 아예 없이 기학습된 모델만 가지고도 condensation 역할을 어느정도 수행할 수 있다는것은 매우 의미 있는 일이다. 하지만 기본적으로 loss가 support vector쪽으로 가게 하기 때문에 mode collapse가 발생할 수 있으며, manifold condition을 추가했음에도 불구하고 Training dataset자체에 대한 접근이 없기 때문에 prior에 대한 정보를 효과적으로 주입하지 못한다. }

 \begin{figure}[t]
  \centering
   \includegraphics[width=0.8\linewidth]{./figures/data_manifold.png}
   \caption{Explanation for overall method}
   \label{fig:data_manifold}
\end{figure}



\subsection{Distribution matching}
\hh{ Dataset에서 전체 데이터 셋을 대표할 수 있는 이미지들을 선별하는 coreset sellection은 data 자체에 대한 훌륭한 representation은 맞지만, 전체 데이터 셋의 분포를 근사하는데에는 부족함이 있었다. training dataset의 분포를 근사할 수 있는 이미지들을 뽑는것이 아니라 생성해야하는 필요성이 있었고,  distribution matching(cite)에서는 어떠한 embeding function을 사용하여 data dimentsion 보다 낮은 dimension에서의 비교를 통해서 효과적으로 이미지들을 synthesize하려고 시도하였다. 기본적으로 DM에서는 real data들과 synthetic data들이 low dimensional embedding space에서 거리를 줄이는 MMD(Maximum mean dicrepancy)를 줄이는 loss 를 apply 하였다 : 
\nj{아래에서도 notation에 대한 설명 필요}
$$\sup_{\|\psi\|_H \leq 1} \left| \mathbb{E}[\psi(S)] - \mathbb{E}[\psi(T)] \right|$$  data distribution 자체에 접근할 수 없으므로 emperical 하게는  $$\min_{\mathbb{E}_{\omega \sim \mathcal{P}} S} \left\| \frac{1}{|T|} \sum_{i=1}^{|T|} \psi(\mathbf{A}(x_i, \omega)) - \frac{1}{|S|} \sum_{j=1}^{|S|} \psi(\mathbf{A}(s_j, \omega)) \right\|^2 .$$를 사용하였다. 위 loss를 사용하여 synthesized dataset과 training dataset간의 embedding 거리를 줄여주어 training dataset의 정보들을 소수의 synthesized된 dataset에 입히려한다.  이때 differentiable Siamese augmentation은 data 자체에 대한 prior knowledge를 학습하기 위해 적용하였으며 위 loss만을 통하여 bi-level optimization과 같은 큰 computational cost를 사용하지 않고도 빠르고 효과적이게 synthesized dataset을 뽑아낼 수 있다.\\ 하지만 위 방식은 initial point를 training dataset에서 뽑아서 사용함으로써 어떤 data를 뽑았느냐에 따라서 영향을 강하게 받고, 뽑은 데이터에 대하여 bias가 있는 상태로 synthesize 된수 있다. 따라서 우리는 bias가 상대적으로 적은 initial point를 utillize할 필요성을 느꼈고 따라서 우리는 DSV를 initial point로 사용하고자 한다. (이거에 대한 실험 필요 : DSV를 initial로 했을때, random image들을 initial로 했을때) }



\section{Method}
\label{sec:method}
\hh{ \textbf{Notations} 이번 섹션에서는 training dataset에 대한 접근이 제한적인 환경에서 semi-supervised learning을 활용하여 효과적으로 condensation을 할 수 있는 방법에 대하여 논한다. class C인 전체 training set T에 대하여 일부의 데이터셋 T' $\{x_i,y_i\}$에만 접근이 가능하며 pretrained 된 모델 $\Phi(\cdot; \theta^*)$를 가지고 있다고 하자. 이때 우리의 목표는 전체 training dataset T의 성능을 낼 수 있는  synthesized dataset S $\{s_j,y_j\}$ 를 만드는 것이다. 이때 class c에 해당하는 T'의 cardinality $|\{x_i|y_i=c\}|$ 를 class 별 접근가능한 데이터수 pipc라고 정의하며, class c에 해당하는 S'의 cardinality $|\{s_j|y_j=c\}|$ 를 class 별 학습가능 데이터수 ipc로 정의한다.  }




\subsection{Distribution matching with DSVs}
\hh{\textbf{DKKT loss} DKKT loss는 dsv들을 올바른 class로 classify하는 primal loss와, decision boundary에 있는 support vector로 수렴하게 하는 stationarity condition으로 구성된다. DSV candidate $x_i$들과 이에 corresponding하는 Lagrange multipliers $\lambda_i$ 들에 그리고 for some multiclassification loss $\L$ 로부터 primal loss 와 stationarity loss는 다음과 같이 표현될 수 있다. 
%
\begin{equation*}\label{eq:two_step_loss}
L_i = 
\begin{cases} 
0 & \text{if } \argmax_c \Phi_c(x_i; \theta^*) = y_i, \\
L(\Phi(x_i; \theta^*), y_i) & \text{otherwise}.
\end{cases}
\end{equation*}
%
%
\begin{equation}\label{eq:total_loss}
L_{\text{primal}} = \frac{1}{n} \sum_{i=1}^n L_i.
\end{equation}
%
%
\begin{equation}\label{eq:stationarity}
L_{\text{stat}} = D(\theta^*, -\sum_{i=1}^n \lambda_i \nabla_\theta L(\Phi(x_i;\theta^*), y_i))
\end{equation}
%
DKKT loss는 primal loss 와 stationary loss의 어떤 weighting factor $\alpha$ 와의 선형결합으로 나타낼 수 있다.
%
\begin{equation}\label{eq:DKKT loss}
L_{\text{DKKT}}(X) = L_{\text{primal}}(X) + \alpha L_{\text{stat}}(X)
\end{equation}
%
}

\hh{\textbf{Dataset matching loss}  $L_{\text{DKKT}}$는 기학습된 모델만을 이용하지만 이는 DSV들을 실제 data distribution으로 보내는데에는 한계가 있다. 따라서 computation을 최소화하면서 DSV들을 좋은 initial point로 하여 synthesized 된 이미지들을 data manifold에 가져다 놓을 필요성이 있다. 우리는 Distribution matching loss를 활용하여, 접근이 가능한 training datset을 anchor로 삼아 효과적으로 synthesized image에 실제 data 정보들을 주입하였다. $L_{\text{dm}}$은 아래와 같다. $$ L_{\text{DM}} = \left\| \frac{1}{|T|} \sum_{i=1}^{|T|} \psi(\mathbf{A}(x_i, \omega)) - \frac{1}{|S|} \sum_{j=1}^{|S|} \psi(\mathbf{A}(s_j, \omega)) \right\|^2 $$\\}
\hh{\textbf{Practical Distribution Matching} Practical Distribution Matching은 기본적으로 $L_{\text{DKKT}}(X)$ 와 $L_{\text{DM}}(X)$의 선형 결합으로 표현한다. 이때 DKKT의 manifold condition인 augmentation invarience 성질까지 사용하여 differentiable augmentation A를 적용한 $L_{\text{DKKT}}(A(X))$ loss도 추가한다. 따라서 최종 total loss는 아래와 같이 표현된다.
%
\begin{equation}\label{eq:Total loss}
L_{\text{Total}}(X) = L_{\text{DKKT}}(X) + \beta L_{\text{DKKT}}(A(X)) +\gamma L_{\text{DM}}(X)
\end{equation}
%
}
onstage synthesis 와 two stage synthesis에 대한 설명,  notation 정리 다시하기, 알고리즘 수정 등등


